Sparse Weight Averaging with Multiple Particles for Iterative Magnitude Pruning

Given the ever-increasing size of modern neural networks, the significance of sparse architectures has surged due to their accelerated inference speeds and minimal memory demands. When it comes to global pruning techniques, Iterative Magnitude Pruning (IMP) still stands as a state-of-the-art algorithm despite its simple nature, particularly in extremely sparse regimes. In light of the recent finding that the two successive matching IMP solutions are linearly connected without a loss barrier, we propose Sparse Weight Averaging with Multiple Particles (SWAMP), a straightforward modification of IMP that achieves performance comparable to an ensemble of two IMP solutions. For every iteration, we concurrently train multiple sparse models, referred to as particles, using different batch orders yet the same matching ticket, and then weight average such models to produce a single mask. We demonstrate that our method consistently outperforms existing baselines across different sparsities through extensive experiments on various data and neural network structures.

==> main/related.tex <==
\section{Related Works}
\label{main:sec:related}

\textbf{Magnitude-based pruning and lottery ticket hypothesis.}
Neural network pruning techniques aim to identify parameters that can be removed from the network without affecting its performance. The simplest yet effective pruning strategy is \textit{magnitude-based pruning}, which involves removing parameters with small magnitudes~\citep{janowsky1989pruning,han2015learning}. While there is no guarantee that zeroing the weights that are close to zero will mitigate the increase in training loss~\citep{lecun1989optimal,hassibi1992second}, magnitude-based pruning can still be effective as it minimizes changes in the output of each layer~\citep{dong2017learning,park2020lookahead}. Empirical studies have demonstrated that \textit{iterative magnitude pruning (IMP)} - applying magnitude-based pruning multiple times - can effectively remove a large proportion of weights in neural networks~\citep{frankle2019lottery,renda2020comparing,frankle2020linear}.

\textbf{Loss landscape and weight averaging.}
Recent studies have shown that the loss landscape of modern deep neural networks exhibits \textit{mode-connectivity}, which means that the local minima found through stochastic optimization are connected by continuous low-loss paths~\citep{draxler2018essentially,garipov2018loss}. It motivates researchers to explore subspaces in the weight space that contain high-performing solutions~\citep{izmailov2020subspace,wortsman2021learning}. One promising approach to obtain such solutions is \textit{weight averaging}, which involves taking the average of weights across multiple points~\citep{izmailov2018averaging,wortsman2022model}. The main assumption of the weight averaging strategy is that all points are located in the same basin of attraction, which may not hold in the case of sparse networks where different sparse structures may correspond to different areas in the loss landscape. However, recent works~\citep{frankle2020linear,evci2022gradient, paul2023unmasking} suggest that this assumption may hold even for sparse networks, as there is a linear connectivity between the solutions of different sparsities obtained through iterative magnitude pruning. As a concurrent work, \cite{yin2023lottery} propose to weight-average the sparse masks generated from consecutive IMP iterations in order to obtain a single stronger sparse network. See \cref{app:sec:related_work} for further literature review on pruning and loss landscape analysis. 


==> table/main_imagenet.tex <==
\begin{table}[t]
\centering
\caption{Classification accuracy on ImageNet. As the official test split of ImageNet is not publicly accessible, ImageNet-V2 serves as a replacement for the test split. The numbers within parentheses indicate the difference from the IMP baseline. For further results, refer to \cref{app:sec:additional_experiments:imagenet}.}
\label{table/main_imagenet}
\setlength{\tabcolsep}{0.5em}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{cllllll}
    \toprule
    & & \multicolumn{5}{c}{Sparsity} \\
    \cmidrule(lr){3-7}
    & Method & 0\% & 48.7\% & 73.6\% & 86.4\% & 92.9\% \\
    \midrule
    \multirow{2}{*}{\Centerstack{ImageNet-Val\\(ResNet-50)}}
    & IMP               & 76.24 & 76.50 & 76.49 & 76.23 & 75.04 \\
    & \bf{SWAMP} & 76.13 \CM{0.11} & 76.87 \CP{0.37} & 76.65 \CP{0.16} & 76.40 \CP{0.17} & 75.34 \CP{0.30} \\
    \midrule
    \multirow{2}{*}{\Centerstack{ImageNet-V2\\(ResNet-50)}}
    & IMP               & 64.29 & 64.10 & 63.83 & 63.08 & 62.17 \\
    & \bf{SWAMP} & 64.10 \CM{0.19} & 64.29 \CP{0.19} & 64.42 \CP{0.59} & 63.97 \CP{0.89} & 62.90 \CP{0.73} \\
    \bottomrule
\end{tabular}}
\end{table}

